Which exceptional low-dimensional projections of a Gaussian point cloud can be found in polynomial time?

Given $d$-dimensional standard Gaussian vectors $\boldsymbol{x}_1,\dots, \boldsymbol{x}_n$, we consider the set of all empirical distributions of its $m$-dimensional projections, for $m$ a fixed constant. Diaconis and Freedman (1984) proved that, if $n/d\to \infty$, all such distributions converge to the standard Gaussian distribution. In contrast, we study the proportional asymptotics, whereby $n,d\to \infty$ with $n/d\to \alpha \in (0, \infty)$. In this case, the projection of the data points along a typical random subspace is again Gaussian, but the set $\mathscr{F}_{m,\alpha}$ of all probability distributions that are asymptotically feasible as $m$-dimensional projections contains non-Gaussian distributions corresponding to exceptional subspaces. Non-rigorous methods from statistical physics yield an indirect characterization of $\mathscr{F}_{m,\alpha}$ in terms of a generalized Parisi formula. Motivated by the goal of putting this formula on a rigorous basis, and to understand whether these projections can be found efficiently, we study the subset $\mathscr{F}^{\rm alg}_{m,\alpha}\subseteq \mathscr{F}_{m,\alpha}$ of distributions that can be realized by a class of iterative algorithms. We prove that this set is characterized by a certain stochastic optimal control problem, and obtain a dual characterization of this problem in terms of a variational principle that extends Parisi's formula. As a byproduct, we obtain computationally achievable values for a class of random optimization problems including `generalized spherical perceptron' models.

==> macros.tex <==
\usepackage{amsmath,amssymb,amsfonts,amsthm,bbm}
%\usepackage[authoryear]{natbib}
\usepackage{verbatim}
\usepackage{setspace}
\usepackage{graphicx}
\usepackage{subcaption}
\usepackage{comment}
\usepackage{enumitem}
\RequirePackage[colorlinks,citecolor=blue,urlcolor=blue,linkcolor=blue,linktocpage=true]{hyperref}
\usepackage[dvipsnames]{xcolor}
\usepackage{bbm}
\usepackage{algpseudocode}
\usepackage{algorithm} 
\usepackage[capitalise]{cleveref}


%%%%%%%%%% define macro conditionals 
\newif\ifStat
\newif\ifNote
\newif\ifComments
\newif\ifThmitalic


\Stattrue
%\Statfalse
%\Notetrue
\Notefalse
%\Commentstrue
%\Commentsfalse
\Thmitalictrue
%\Thmitalicfalse




\ifStat
\renewcommand{\hat}{\widehat}
\renewcommand{\tilde}{\widetilde}
\renewcommand{\bar}{\overline}
\else

\fi



%%%%%%%%%% page setup %%%%%%%%%%
%\textheight 8.5 in
%\textwidth 6.5 in
%\topmargin -0.5 in
%\oddsidemargin -0.1 in

\usepackage[top=1in, bottom=1in, left=1in, right=1in]{geometry}


\makeatletter
\newcommand*{\rom}[1]{\expandafter\@slowromancap\romannumeral #1@}
\makeatother

\newcommand{\eqi}[1]{\mathrel{\overset{\makebox[0pt]{\normalfont\scriptsize\sffamily (#1)}}{=}}}
\newcommand{\lei}[1]{\mathrel{\overset{\makebox[0pt]{\normalfont\scriptsize\sffamily (#1)}}{\le}}}
\newcommand{\gei}[1]{\mathrel{\overset{\makebox[0pt]{\normalfont\scriptsize\sffamily (#1)}}{\ge}}}
\newcommand{\lessi}[1]{\mathrel{\overset{\makebox[0pt]{\normalfont\scriptsize\sffamily (#1)}}{\lesssim}}}
\newcommand{\gtri}[1]{\mathrel{\overset{\makebox[0pt]{\normalfont\scriptsize\sffamily (#1)}}{\gtrsim}}}
\newcommand{\<}{\langle}
\renewcommand{\>}{\rangle}

%\newcommand{\conv}{\mathrm{conv}}

\def\FS{{\mathscr{L}}}
\def\FSG{{\mathscr{L}_{\#}}}

\newcommand{\diag}{\mathrm{diag}}
\newcommand{\diagg}{\mathrm{diagg}}
\newcommand{\rank}{\mathrm{rank}}
\newcommand{\spann}{\mathrm{span}}
\newcommand{\supp}{\mathrm{supp}}
\newcommand{\sgnn}{\mathrm{sign}}
\newcommand{\sgn}{\mathrm{sgn}}
\newcommand{\sign}{\mathrm{sign}}
\newcommand{\conv}{\mathrm{conv}}
\newcommand{\cov}{\mathrm{Cov}}
\newcommand{\var}{\mathrm{Var}}
\newcommand{\trace}{\mathrm{trace}}
\newcommand{\Tr}{\mathrm{Tr}}
\newcommand{\vect}{\mathrm{Vec}}
\newcommand{\RE}{\mathrm{RE}}
\newcommand{\GMM}{\mathrm{GMM}}
\newcommand{\LHS}{\mathrm{LHS}}
\newcommand{\RHS}{\mathrm{RHS}}
\newcommand{\minimize}{\mbox{minimize}}
\newcommand{\st}{\mbox{subject to}}
\newcommand{\argmin}{\mbox{argmin}}
\newcommand{\svd}{\mathrm{svd}}
\newcommand{\eigen}{\mathrm{eigen}}
\newcommand{\op}{\mathrm{op}}
\newcommand{\sam}{\mathrm{sam}}
\newcommand{\KL}{\normalfont \mathrm{\texttt{KL}}}
\newcommand{\Bern}{\mathrm{Bern}}
\newcommand{\row}{\mathrm{row}}
\newcommand{\col}{\mathrm{col}}
\newcommand{\where}{\text{where}}
\newcommand{\mle}{\mathrm{MLE}}
\newcommand{\iid}{\mathrm{i.i.d.}}
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\thh}{\text{th}}
\newcommand{\res}{\mathrm{res}}
\newcommand{\polylog}{\mathrm{polylog}}
\newcommand{\poly}{\mathrm{poly}}
\newcommand{\Unif}{\mathrm{Unif}}
\newcommand{\dist}{\mathrm{dist}}
\newcommand{\low}{\mathrm{low}}
\newcommand{\high}{\mathrm{high}}
\newcommand{\init}{\mathrm{init}}
\newcommand{\Law}{\mathrm{Law}}
\newcommand{\kz}[1]{\noindent{{\color{red}\textbf{\#\#\# KZ:} \textsf{#1} \#\#\#}}}
\DeclareMathOperator*{\argmax}{\mbox{argmax}}










\newcommand{\norm}[1]{\left\|{#1}\right\|}

\newcommand{\Q}{\mathbb{Q}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\bbS}{\mathbb{S}}
\newcommand{\E}{\mathbb{E}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\bfR}{\mathbf{R}}
\newcommand{\calA}{\mathcal{A}}
\newcommand{\veps}{\varepsilon}

\renewcommand{\O}{\mathcal{O}}
\renewcommand{\P}{\mathbb{P}}
\renewcommand{\S}{\mathbb{S}}
\renewcommand{\d}{\mathrm{d}}

%% boldface

\newcommand{\bff}{\mathrm{\bf f}}
\newcommand{\ba}{\mathrm{\bf a}}
\newcommand{\be}{\mathrm{\bf e}}
\newcommand{\bh}{\mathrm{\bf h}}
\newcommand{\br}{\mathrm{\bf r}}
\newcommand{\bs}{\mathrm{\bf s}}
\newcommand{\bt}{\mathrm{\bf t}}
\newcommand{\bu}{\mathrm{\bf u}}
\newcommand{\bv}{\mathrm{\bf v}}
\newcommand{\bw}{\mathrm{\bf w}}
\newcommand{\bx}{\mathrm{\bf x}}

\newcommand{\by}{\mathrm{\bf y}}
\newcommand{\bz}{\mathrm{\bf z}}
\newcommand{\bA}{\mathrm{\bf A}}
\newcommand{\bB}{\mathrm{\bf B}}
\newcommand{\bZ}{\mathrm{\bf Z}}
\newcommand{\bC}{\mathrm{\bf C}}
\newcommand{\bD}{\mathrm{\bf D}}
\newcommand{\bE}{\mathrm{\bf E}}
\newcommand{\bF}{\mathrm{\bf F}}
\newcommand{\bK}{\mathrm{\bf K}}
\newcommand{\bO}{\mathrm{\bf O}}
\newcommand{\bT}{\mathrm{\bf T}}
\newcommand{\bW}{\mathrm{\bf W}}
\newcommand{\bG}{\mathrm{\bf G}}
\newcommand{\bM}{\mathrm{\bf M}}
\newcommand{\bH}{\mathrm{\bf H}}
\newcommand{\bI}{\mathrm{\bf I}}
\newcommand{\bg}{\mathrm{\bf g}}
\newcommand{\bP}{\mathrm{\bf P}}
\newcommand{\bV}{\mathrm{\bf V}}
\newcommand{\bQ}{\mathrm{\bf Q}}
\newcommand{\bR}{\mathrm{\bf R}}
\newcommand{\bS}{\mathrm{\bf S}}
\newcommand{\bU}{\mathrm{\bf U}}
\newcommand{\bX}{\mathrm{\bf X}}
\newcommand{\bY}{\mathrm{\bf Y}}
\newcommand{\bL}{\mathrm{\bf L}}


\newcommand{\oxx}{\overline{\boldsymbol x}}
\newcommand{\xx}{\text{\boldmath $x$}}
\renewcommand{\AA}{\text{\boldmath $A$}}
\newcommand{\BB}{\text{\boldmath $B$}}
\newcommand{\GG}{\text{\boldmath $G$}}
\newcommand{\XX}{\text{\boldmath $X$}}
\newcommand{\MM}{\text{\boldmath $M$}}
\newcommand{\CC}{\text{\boldmath $C$}}
\newcommand{\yy}{\text{\boldmath $y$}}
\newcommand{\zz}{\text{\boldmath $z$}}
\newcommand{\ww}{\text{\boldmath $w$}}
\newcommand{\YY}{\text{\boldmath $Y$}}
\newcommand{\ZZ}{\text{\boldmath $Z$}}
\newcommand{\WW}{\text{\boldmath $W$}}
\newcommand{\VV}{\text{\boldmath $V$}}
\newcommand{\UU}{\text{\boldmath $U$}}
\newcommand{\vv}{\text{\boldmath $v$}}
\newcommand{\RR}{\text{\boldmath $R$}}
\newcommand{\uu}{\text{\boldmath $u$}}
\newcommand{\bss}{\text{\boldmath $s$}}
\newcommand{\uI}{\text{\boldmath $u_I$}}
%\newcommand{\bzero}{\text{\boldmath $0$}}
\newcommand{\II}{\text{\boldmath $I$}}
\renewcommand{\aa}{\text{\boldmath $a$}}
\newcommand{\bb}{\text{\boldmath $b$}}
\newcommand{\cc}{\text{\boldmath $c$}}
\newcommand{\ee}{\text{\boldmath $e$}}
\newcommand{\ff}{\text{\boldmath $f$}}
\newcommand{\kk}{\text{\boldmath $k$}}
\newcommand{\nn}{\text{\boldmath $n$}}
\newcommand{\bgg}{\text{\boldmath $g$}}
\newcommand{\pp}{\text{\boldmath $p$}}
\newcommand{\rr}{\text{\boldmath $r$}}
\newcommand{\hh}{\text{\boldmath $h$}}
%\newcommand{\qq}{\text{\boldmath $q$}}
\newcommand{\QQ}{\text{\boldmath $Q$}}
\newcommand{\bGG}{\text{\boldmath $G$}}

\newcommand{\vveps}{{\boldsymbol \varepsilon}}

\def\JF{{J_F}}

\newcommand{\tWW}{\tilde{\text{\boldmath $W$}}}
\newcommand{\tVV}{\tilde{\text{\boldmath $V$}}}

\newcommand{\balpha}{\text{\boldmath $\alpha$}}
\newcommand{\bm}{\text{\boldmath $m$}}
\newcommand{\bpi}{\text{\boldmath $\pi$}}
\newcommand{\bbeta}{\text{\boldmath $\beta$}}
\newcommand{\bdelta}{\text{\boldmath $\delta$}}
\newcommand{\btheta}{\text{\boldmath $\theta$}}
\newcommand{\bDelta}{\text{\boldmath $\Delta$}}
\newcommand{\bone}{\mathrm{\bf 1}}
\newcommand{\bzero}{\mathrm{\bf 0}}
\newcommand{\bet}{\text{\boldmath $\eta$}}
\newcommand{\bxi}{\text{\boldmath $\xi$}}
\newcommand{\bveps}{\text{\boldmath $\varepsilon$}}
\newcommand{\bmu}{\text{\boldmath $\mu$}}
\newcommand{\bLambda}{\text{\boldmath $\Lambda$}}
\newcommand{\blambda}{\text{\boldmath $\lambda$}}
\newcommand{\bgamma}{\text{\boldmath $\gamma$}}
\newcommand{\bGamma}{\text{\boldmath $\Gamma$}}
\newcommand{\bkappa}{\text{\boldmath $\kappa$}}
\newcommand{\bTheta}{\text{\boldmath $\Theta$}}
\newcommand{\bsigma}{\text{\boldmath $\sigma$}}
\newcommand{\bSigma}{\text{\boldmath $\Sigma$}}
\newcommand{\bOmega}{\text{\boldmath $\Omega$}}
\newcommand{\bomega}{\text{\boldmath $\omega$}}
\newcommand{\bPhi}{\text{\boldmath $\Phi$}}
\newcommand{\bXi}{\text{\boldmath $\Xi$}}
\newcommand{\bPsi}{\text{\boldmath $\Psi$}}
\newcommand{\bPi}{\text{\boldmath $\Pi$}}
\newcommand{\bepsilon}{\text{\boldmath $\epsilon$}}

\newcommand{\cI}{\mathcal{I}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cD}{\mathcal{D}}
\newcommand{\cK}{\mathcal{K}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cS}{\mathcal{S}}
\newcommand{\cL}{\mathcal{L}}
\newcommand{\cV}{\mathcal{V}}
\newcommand{\cJ}{\mathcal{J}}
\newcommand{\cR}{\mathcal{R}}
\newcommand{\cU}{\mathcal{U}}
\newcommand{\cO}{\mathcal{O}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cA}{\mathcal{A}}
\newcommand{\cP}{\mathcal{P}}
\newcommand{\cX}{\mathcal{X}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cE}{\mathcal{E}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\cT}{\mathcal{T}}
\newcommand{\cW}{\mathcal{W}}
\newcommand{\wtilde}{\widetilde}

\def\close{\mathrm {cl} \ }
\def\VH{\mathscr{V}}
\def\oVH{\overline{\mathscr{V}}}
\def\sA{\mathsf{A}}
\def\cuC{\mathscr{C}}
\def\cuX{\mathscr{X}}
\def\cuY{\mathscr{Y}}
\def\cuE{\mathscr{E}}
\def\cuF{\mathscr{F}}
\def\cuP{\mathscr{P}}
\def\cuS{\mathscr{S}}
\def\cuQ{\mathscr{Q}}
\def\cuG{\mathscr{G}}
\def\normal{{\sf N}}
\def\id{{\boldsymbol I}}
\def\RI{{\rm RI}}

\def\MAX{{\sf M}}
\def\BV{{\rm BV}}

\def\de{{\rm d}}
\newcommand{\sN}{\mathsf{N}}
\newcommand{\sB}{\mathsf{B}}
\def\sTV{\mbox{\scriptsize\rm TV}}
\def\sKS{\mbox{\scriptsize\rm KS}}
\def\sKL{\mbox{\scriptsize\rm KL}}
\def\sAMP{\mbox{\tiny\rm AMP}}
\def\lod{\underline{d}}
\def\eps{\varepsilon}
\def\Lip{\mbox{\tiny\rm Lip}}

\def\salg{\mbox{\scriptsize\rm alg}}

\def\hV{\widehat{V}}
\def\sV{{\sf V}}
\def\sT{{\sf T}}
\def\sF{\mathsf{F}}
\def\SFu{{\sf SF}}

\DeclareMathOperator*{\plimsup}{p-lim\, sup}
\DeclareMathOperator*{\pliminf}{p-lim\, inf}
\DeclareMathOperator*{\plim}{p-lim}

\newcommand{\am}[1]{\textcolor{red}{\bf [Andrea:  #1]}}


\newcommand{\hb}{\widehat \bb}
\newcommand{\hE}{\widehat \bE}
\newcommand{\hF}{\widehat \bF}
\newcommand{\hf}{\widehat \bff}
\newcommand{\hR}{\widehat R}
\newcommand{\hG}{\widehat \bG}
\newcommand{\hu}{\widehat \bu}
\newcommand{\hvar}{\widehat \var}
\newcommand{\hcov}{\widehat \cov}
\newcommand{\hbveps}{\widehat\bveps}
\newcommand{\heps}{\widehat\beps}
\newcommand{\hSig}{\widehat\Sig}
\newcommand{\tSig}{\widetilde\Sig}
\newcommand{\hsig}{\widehat\sigma}
\newcommand{\hlam}{\widehat\lambda}
\newcommand{\hbeta}{\widehat\beta}
\newcommand{\hLam}{\widehat \bLambda}
\newcommand{\hmu}{\widehat\bmu}
\newcommand{\hxi}{\widehat\bxi}
\newcommand{\Sig}{\mathbf{\Sigma}}
\newcommand{\hw}{\widehat \bw}
\newcommand{\wt}{\widetilde}


\def\sUB{\mbox{\tiny\rm UB}}
\def\sLB{\mbox{\tiny\rm LB}}


%% for editting


\newcommand{\RMK}[1]{{\color{blue}{[Comment: #1]}}}
\newcommand{\TODO}[1]{{\color{red}{[#1]}}}
\newcommand{\rmk}[1]{{\color{blue}{[#1]}}}


\ifNote

%\numberwithin{equation}[section]
\theoremstyle{plain}
\newtheorem{thm}{Theorem}
\newtheorem{claim}{Claim}
\newtheorem{defn}{Definition}
\newtheorem{lem}{Lemma}
\newtheorem{cor}[lem]{Corollary}
\newtheorem{prop}[lem]{Proposition}
\newtheorem{ass}{Assumption}
\newtheorem{fact}{Fact}
\theoremstyle{definition}
\newtheorem{exm}{Example}
\newtheorem{rem}{Remark}
\newtheorem{conj}{Conjecture}

\else\ifThmitalic

\newtheorem{thm}{Theorem}[section]
\newtheorem{claim}{Claim}[section]
\newtheorem{defn}{Definition}
\newtheorem{lem}{Lemma}[section]
\newtheorem{cor}[lem]{Corollary}
\newtheorem{prop}[lem]{Proposition}
\newtheorem{ass}{Assumption}[section]
\newtheorem{fact}{Fact}
\newtheorem{conj}{Conjecture}[section]
\theoremstyle{definition}
\newtheorem{rem}{Remark}
\newtheorem{exm}{Example}

\else

\fi
\fi




